Trajectory Prediction for Autonomous Driving with Topometric Map

State-of-the-art autonomous driving systems rely on high definition (HD) maps for localization and navigation. However, building and maintaining HD maps is time-consuming and expensive. Furthermore, the HD maps assume structured environment such as the existence of major road and lanes, which are not present in rural areas. In this work, we propose an end-to-end transformer networks based approach for map-less autonomous driving. The proposed model takes raw LiDAR data and noisy topometric map as input and produces precise local trajectory for navigation. We demonstrate the effectiveness of our method in real-world driving data, including both urban and rural areas. The experimental results show that the proposed method outperforms state-of-the-art multimodal methods and is robust to the perturbations of the topometric map. The code of the proposed method is publicly available at \url{https://github.com/Jiaolong/trajectory-prediction}.

==> sections/table_ablation.tex <==
\begin{table}
    \small
    \centering
\begin{tabular}{cllcccccc}
    \toprule
    Model    & FDE$\downarrow$  & \ade{1} $\downarrow$ & \ade{2} $\downarrow$ & \ade{3} $\downarrow$ & \hitrate{1} $\uparrow$ & \hitrate{2} $\uparrow$ & \hitrate{3} $\uparrow$ \\
    \midrule
    M0       &   0.64  & 0.30  & 0.24 & 0.23 & 0.95  & 0.97 & 0.97  \\
    \midrule
    M1   &   0.80  & 0.34 & 0.30 & 0.26  & 0.91 & 0.95 & 0.97  \\
    \midrule
    M2   &   0.87  & 0.35 & 0.29  & 0.23  & 0.91 & 0.95 & 0.98 \\
    M3   &   0.66  & 0.31 & 0.25 & 0.25   & 0.95 & 0.97 & 0.98    \\ 
    \midrule  
    M4        & 0.78 & 0.32 & 0.28 & 0.24 & 0.93 & 0.95 & 0.96 \\     
    \bottomrule
\end{tabular}
\caption{Ablation studies on KITTI-10.}
\label{tab:ablation}
\end{table}

==> sections/table_pertubation.tex <==
\begin{table}[ht]
    \small
    \centering
    \begin{tabular}{llcc}
    \toprule
    Perturbation    & FDE$\downarrow$  & \ade{1} $\downarrow$ & \hitrate{1} $\uparrow$\\
    \midrule
    0.0 m       &   0.64            & 0.30                  & 0.95  \\
    \midrule
    1.0 m   &   0.66$\pm$0.01       & 0.31$\pm$0.01         & 0.95$\pm$0.01  \\
    3.0 m  &   0.79$\pm$0.04       & 0.36$\pm$0.02         & 0.92$\pm$0.01  \\
    5.0 m  &   1.07$\pm$0.04       & 0.51$\pm$0.01         & 0.86$\pm$0.01  \\
    \bottomrule
    \end{tabular}
    \caption{Robustness of the model under different lateral perturbations to the topometric map.}
    \label{tab:perturbation}
\end{table}

==> sections/table_results.tex <==
\begin{table*}
    %\small
    \centering
    \begin{tabular}{cllcccccc}
    \toprule
    Dataset                         &Method    & FDE$\downarrow$  & \ade{1} $\downarrow$ & \ade{2} $\downarrow$ & \ade{3} $\downarrow$ & \hitrate{1} $\uparrow$ & \hitrate{2} $\uparrow$ & \hitrate{3} $\uparrow$ \\
    \midrule
    \multirow{2}{*}{KITTI-08}      & CoverNet &   1.28           & 0.62                 & 0.47                 & \textbf{0.41}                 & 0.80                   & 0.84                 & 0.87  \\
    &                          MTP     &   1.06           & 0.53                 & 0.45                 & 0.42                 & \textbf{0.85}                   & \textbf{0.88}                 & \textbf{0.89}  \\
    &                          MultiPath       &   \textbf{1.00}    & \textbf{0.51}     & \textbf{0.44}                 & \textbf{0.41}                 & \textbf{0.85}                   & 0.86                 & \textbf{0.89}  \\

    \midrule
    \multirow{2}{*}{KITTI-09}      & CoverNet &   1.42           & 0.56                 & 0.38                 & 0.33                 & 0.71                   & 0.86                 & 0.91  \\
    &                          MTP     &   0.95           & 0.39                 & 0.29                 & 0.25                 & 0.87                   & \textbf{0.94}                 & \textbf{0.96}  \\
    &                          MultiPath       &   \textbf{0.85}  & \textbf{0.35}  & \textbf{0.27}  & \textbf{0.23}    & \textbf{0.90}                   & \textbf{0.94}                 & \textbf{0.96}  \\

    \midrule
    \multirow{3}{*}{KITTI-10}     & Const. vel. \& yaw &   2.11           & 0.90                 & 0.90                 & 0.90                 & 0.64                   & 0.64                 & 0.64  \\ 
    & CoverNet &   1.36           & 0.53                 & 0.37                 & 0.30                 & 0.78                   & 0.89                 & 0.94  \\
    &                          MTP     &   0.73           & 0.31                 & 0.26                 & \textbf{0.23}    & 0.93                   & \textbf{0.97}                 & \textbf{0.97}  \\
    &                          MultiPath       &   \textbf{0.64}  & \textbf{0.30}  & \textbf{0.24} & \textbf{0.23} & \textbf{0.95}     & \textbf{0.97}                 & \textbf{0.97}  \\

    \midrule
    \multirow{3}{*}{Rural}      & CoverNet &   2.69           & 1.37                 & 0.96                 & 0.78                 & 0.65                   & 0.75                & 0.79  \\
    &                          MTP     &   1.61           & \textbf{0.84}    & \textbf{0.71}        & \textbf{0.66}        & \textbf{0.76}          & \textbf{0.82}       & \textbf{0.82}  \\
    &                          MultiPath       &   1.59  & 0.90             & 0.75                 & 0.71                 & 0.75                   & 0.81                & \textbf{0.82}  \\
    &                          Ours       &   \textbf{1.19}  & \textbf{0.69}             & 0                 & 0                 & \textbf{0.85}                   & 0                & 0  \\
    \bottomrule
    \end{tabular}
    \caption{Results on KITTI and our collected rural scene dataset. Smaller minADE\textsubscript{k} and FDE is better. Larger \hitrate{k} is better.}
    \label{tab:results}
\end{table*}

